Theoretical Perspectives on Deep Learning Methods in Inverse Problems

In recent years, there have been significant advances in the use of deep learning methods in inverse problems such as denoising, compressive sensing, inpainting, and super-resolution. While this line of works has predominantly been driven by practical algorithms and experiments, it has also given rise to a variety of intriguing theoretical problems. In this paper, we survey some of the prominent theoretical developments in this line of works, focusing in particular on generative priors, untrained neural network priors, and unfolding algorithms. In addition to summarizing existing results in these topics, we highlight several ongoing challenges and open problems.

==> figs/untrained_OLD.tex <==

\newcommand{\reals}{\mathbb R}
\newcommand{\mB}{\mathbf{B}} 
\newcommand{\mC}{\mathbf{C}}
\newcommand{\mU}{\mathbf{U}}
\newcommand{\mA}{\mathbf{A}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}

\newcommand{\veta}{{\bm \eta}}
\newcommand{\vtheta}{{\bm \theta}}
\newcommand{\mTheta}{{\bm \Theta}}


\newcommand{\cn}{\mathrm{cn}}
\newcommand{\relu}{\mathrm{relu}}
\newcommand{\kout}{q}


%%%
\section{Signal reconstruction with Untrained Neural Networks} \label{sec:untrained} 


Un-trained neural networks have very recently emerged as a highly successful alternative to trained methods for image recovery and restoration, for a variety of problems including denoising~\cite{ulyanov_DeepImagePrior_2018,heckel_DeepDecoderConcise_2019} and signal reconstruction from few or noisy images~\cite{yoo_TimeDependentDeepImage_2021,vanveen_CompressedSensingDeep_2018,jagatap_AlgorithmicGuaranteesInverse_2019,bostan_DeepPhaseDecoder_2020,wang_PhaseImagingUntrained_2020,hyder_GenerativeModelsLowDimensional_2020}. 
%This development has started with~\citet{ulyanov_DeepImagePrior_2018}'s work, which shows that simply fitting an un-trained network with auto-encoder or U-net~\cite{ronneberger_UNetConvolutionalNetworks_2015} architecture to a noisy image denoises that image. 

Un-trained neural networks are a class of image reconstruction methods that, rely on neural networks acting as an image prior without any training and solely based on the architecture of the network and the optimization procedure used to fit them. 

%as opposed to trained neural networks, that learn an image prior from training data, un-trained (convolutional) 

This class of methods emerged when the Deep Image Prior (DIP) paper~\cite{ulyanov_DeepImagePrior_2018}. 
\cite{ulyanov_DeepImagePrior_2018} observed that `training' a standard convolutional auto-encoder (the popular U-net~\cite{ronneberger_UNetConvolutionalNetworks_2015}) on a single noisy image and regularizing by early stopping, enables excellent denoising performance. 

While this class of methods is based on neural networks, it is conceptually also related to sparsity based methods, in that it relies on hand-crafted signal models (neural networks in this case), and is not data driven. However, un-trained networks improve over sparsity-based methods, for example un-trained neural networks give better image quality than sparsity based methods for accelerated magnetic resonance imaging~\cite{darestani_AcceleratedMRIUnTrained_2021}. 

In this section, we first discuss how signal recovery with un-trained neural networks work, and then discuss the existing theory behind it. 

%Convolutional neural networks incorporate implicit assumptions about the signals they generate, such as pixels that are close being related. This makes them particularly well suited for modeling distributions of images, and for representing individual images. 
%As we see in this section, those prior assumptions build into the architecture are so strong that convolutional neural networks are useful tools for image recovery even without ever being exposed to training data.
%Thus, the deep decoder does not use learned or trainable convolutional filters like conventional convolutional networks do, and instead only uses convolutions with fixed convolutional kernels to generate an image.




\subsection{Background}

Recall that our goal is to reconstruct and image $\vx^n$ from a noisy observation $\vy = \mA \vx + \veta \in \reals^m$. Let $G \colon \reals^p \to \reals^n$ be a generative convolutional neural network with parameters $\vtheta \in \reals^p$ and a fixed, randomly chosen input, that's our un-trained network. 
Note that unlink in the previous section, we view the network mapping from its parameter space to its output, and not from the network input to its output. The input of the network is chosen as a random input volume that is fixed and thus part of the network. 
The architecture of the network is critical and discussed in more detail later, for now we note that a good choice is a simple five layer convolutional network. 
We reconstruct an image by initializing the parameters of the network, $\vtheta$, randomly, and then we apply gradient descent to the least-squares loss
\begin{align}
\label{eq:untrainedoptprob}
\mathcal L(\vtheta) = \norm{ \mA G(\vtheta) - \vy }^2_2,
\end{align}
Gradient descent, possibly with early-stopped iterations for regularization, yields the estimate $\hat \vtheta$, from which we estimate the unknown signal as $\hat \vx = G(\hat \vtheta)$.
Again, we note that we are optimizing over the weights of the network not over the input of the network (as in the previous section on signal reconstruction with generative priors). 

This method is based on the empirical observation that un-trained convolutional auto-decoders fit a single natural image faster when optimized with gradient descent than pure noise. 

For this method to work, the architecture, training, and regularization (early stopping here) is critical. 

{\bf Deep image prior: }
Ulyanov et al.~\cite{ulyanov_DeepImagePrior_2018} first observed that using a a standard convolutional auto-encoder (the popular U-net~\cite{ronneberger_UNetConvolutionalNetworks_2015}) as a generator network, and regularizing with early stopping, enables excellent denoising performance. 

{\bf Deep decoder: }
However, many elements of an auto-encoder, are irrelevant for this effect: A more recent paper~\cite{heckel_DeepDecoderConcise_2019} proposed a much simpler image generating network, termed the deep decoder. 
This network can be seen as the relevant part of a convolutional generator architecture to function as an image prior, and can be obtained from a standard convolutional autoencoder by removing the encoder, the skip connections, and perhaps most notably, the trainable convolutional filters of spatial extent larger than one.

%The deep decoder is a convolutional network that consists of one-times-one convoluions 
% RH: have the architecture of the deep decoder in detail here?


%%%
%\paragraph{Convolutional generators}
%\label{sec:untrainedconv}
%A convolutional generator $G \colon \reals^p \to \reals^n$ is a network that takes an input tensor and maps the input tensor to a signal through convolutional operations and applications of non-linearities. Here, we describe a convolutional generator, called deep decoder, that uses \emph{fixed} convolutional only. Fixed convolutional operations are critical for a convolutional generator to function as an image model. 
%
%Let $\mB_0 \in \reals^{n_0 \times k}$ the input volume. Throughout, the input volume is chosen randomly (from a Gaussian distribution) and is fixed. The channels in the $(i+1)$-th layer are given by 
%\[
%\mB_{i+1} = \cn(\relu(\mU_i\mB_i \mC_i )), 
%\quad i = 0, \ldots, d-1,
%\]
%and finally, the output of the $d$-layer network is formed as
%\[
%\vx = %\mathrm{sigmoid}(\mB_d \mC_{d+1}).
%\mB_d \mC_{d+1} \in \reals^{n \times \kout},
%\]
%with $\kout=1$ for a grayscale image, and $\kout =3$ for an image with three color channels.  
%Here, $n_i$ is an integer if the network generates a one-dimensional signal, and $n_i = w_i \times h_i$, if the networks generates an image of width $w$ and height $h$, which is a two-dimensional signal.
%The coefficient matrices $\mC_i \in \reals^{k \times k }$ and $\mC_{d+1} \in \reals^{k \times k}$ contain the weights of the network, and we denote with $\mC$ the set of all those weight parameters. 
%The number of channels, $k$, determines the number of weight parameters of the network, which is $d k^2 + \kout k$; choosing $k$ larger increases the number of parameters of the channels. A typical value for the depth is $d=5$. 
%
%Each column of the tensor $\mB_i \mC_i \in \reals^{n_i \times k}$ is formed by taking linear combinations of the channels of the tensor $\mB_i$ in a way that is consistent across all pixels. In deep learning language, this is often called a $1\times 1$ because it is a degenerate convolution with kernel $1\times 1$ for images. 
%%and the ReLU activation function is given by $\relu(t)=\max(0,t)$. In deep learning, this 
%
%The operator $\mU_i \in \reals^{n_{i+1} \times n_i}$ is a transposed convolution with a fixed convolutional kernel which is chosen as a triangular kernel. Thus, the operation performs bi-linear 2x upsampling. 
%%(this is the standard implementation in the popular software packages pytorch and tensorflow). 
%%As mentioned earlier this convolution with a \emph{fixed kernel} is critical for fitting natural images faster than complex ones.
%
%Finally, $\cn(\cdot)$ performs the channel normalization operation which normalizes each channel individually and can be viewed as a special case of the popular batch normalization operation~\cite{ioffe_BatchNormalizationAccelerating_2015}. 
%This is the least important element of the architecture for the conceptual understanding of the architecture, and can be viewed as a tool for enabling efficient optimization of the network. 
%
%%In its simplest form, channel normalization is defined as follows. Let $\mZ \in \reals^{n\times k}$ be a volume, and let $\vz_i$ be the $i$-th channel of this volume. Then channel normalization performs the operation $\cn(\mZ)_j = \frac{ \vz_{j} - \mathrm{mean}(\vz_{j})  }{ \sqrt{ \mathrm{var}(\vz_{j}) +\epsilon}} \gamma_{j} + \beta_{j}$, where $\mathrm{mean}$ and $\mathrm{var}$ compute the empirical mean and variance, and $\gamma_{j}$ and $\beta_{j}$ are parameters either learned independently for each channel, or are fixed to $1$ and $0$, respectively. The parameter $\epsilon$ is a fixed small constant, for numerical stability. Learning the parameters $\gamma$ and $\beta$ helps the optimization but is not critical. 
%
%
%\begin{itemize}
%    \item Deep image prior \cite{ulyanov2018deep}
%    \item Deep decoder \cite{heckel2019deep}
%\end{itemize}

\subsection{Theory}

Un-trained neural networks enable provable denoising and signal reconstruction from few measurements. Here, we will discuss those guarantees along with intuition why and when un-trained neural networks enable signal reconstruction.

%{\bf Under-parameterized un-trained neural networks.}.
\subsubsection{\bf Under-parameterized un-trained neural networks}
We say that an un-trained neural network is under-parameterized if it has fewer parameters (i.e., the dimensions of the parameter vector $\vtheta$) than it's output dimension, $n$. 
Un-trained networks enable signal reconstruction in the under- and over-parameterized regime. 
We start with discussing the under-parameterized setup first, since it is conceptually simpler. 

The deep decoder~\cite{} is an neural network that transforms an random input volume $\mB_0$ to an output image by applying convolutions with a fixed convolutional up-sampling kernel followed by weighted linear combinations of the channels, followed by relu-nonlinearities, and repeating those operations about five times, to obtain a five layer network. 
For concreteness, a two-layer network is
\begin{align}
\label{eq:twolayerDD}
G(\vtheta) = \relu( \mU_0\mB_0 \mTheta_0 ) \vtheta_1,
\end{align}
where $\mU_0$ is a linear operator implementing a convolution with a fixed upsampling operator, and $\mTheta_0 \in \mathbb R^{k\times k}$ is a parameter matrix forming linear combinations of the channels $\mU_0\mB_0$. Finally, we apply a ReLU non-linearity and again form linear combinations through multiplication with the parameter vector $\vtheta_1$, which yields the output image. The parameters of the network are the weights $\vtheta = (\mTheta_0,\vtheta_1)$.

A five layer version of the network is a concise image model, in that in can represent a natural image with much fewer network parameters than it has pixels. 
Specifically, Figure~1 in the paper~\cite{} shows that representing (or compressing) natural images with a deep decoder that has 30 times fewer parameters than weights gives only a small loss in image quality. 
The loss in image quality is on average less than when compressing images with a sparse wavelet representation, which is known to perform well for image compression, and is the base for the JPEG2000 compression standard.

To summarize, the deep decoder can represent a natural image with very few parameters. At the same time, in the underparameterized regime, it cannot represent much random noise: a $n$-dimensional Gaussian noise vector requires about $p$ parameter to represent a fraction of $p/n$ of its energy. 
As formalized in the following proposition, the deep decoder with $p$ parameters can only represent a fraction $p/n$ of the noise energy:
\begin{proposition}[Prop.~1 in~\cite{}]
Consider the two layer deep decoder~\eqref{eq:twolayerDD} with $p$ parameters and arbitrary upsampling and input matrices. Let $\veta$ be zero-mean Gaussian noise with identity co-variance matrix Then, with high probability,
\begin{align}
\min_{\vtheta} \norm{G(\vtheta) - \veta}_2^2 \geq \norm{\veta}_2^2 \left( 1 - c \frac{p}{n} \right),
\end{align}
where $c$ is a constant hiding a $\log(n)$ term. 
\end{proposition}

Thus, when fitting an underparamerized deep decoder to a noisy image (by minimizing the loss in equation~\ref{eq:untrainedoptprob}), we expect that most of the image is fitted, but only little of the noise, which enables denoising a signal. 
The number of parameters of the network, $p$, is a hyperparameter that trades off how well the network fits the signal or image to be recovered (larger is better) and how much noise it fits (smaller is better). 

Similarly, an under-parameterized un-trained neural network enables reconstruction of a signal from few measurements since if the network is sufficiently underparameterized, there is only one signal that is consistent with the measurements. 

%%%

\subsubsection{\bf Over-parameterized un-trained neural networks}

In the previous section we saw that an under-parameterized un-trained neural network enables image denoising and image reconstruction from few and noisy examples because particular convolutional networks are concise image models. Next, we discuss denoising and image reconstruction with an over-parameterized un-trained network. 

A sufficiently over-parameterized convolutional neural network can fit any single image perfectly, including noise. Thus at first sight is is perhaps surprising that an over-parameterized un-trained network enables signal reconstruction. 

An over-parameterized convolutional network enables signal reconstruction since, when trained with gradient descent, it fits a natural image faster than noise. 
This is illustrated in Figure~\ref{fig:fittingcurves}, where we apply gradient descent to fitting a clean image (Fig.~\ref{fig:fittingcurves}(b)) and noise (Fig.~\ref{fig:fittingcurves}(c)), via minimizing the least-squares loss~\eqref{eq:untrainedoptprob} with $\mA=\mI$ with gradient descent. While after about $3e2$ iterations the network fits the clean example image perfectly, it requires $3e4$ iterations to fit the noise perfectly. If we apply gradient descent to fitting a noisy image (Fig.~\ref{fig:fittingcurves}(a)), the network first fits the image part of the noisy image and only later the noise part of the noisy image. Thus, early stopping the iterations at about $3e2$ iterations denoises the image.


\begin{figure}[t]
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tikzpicture}
\pgfplotsset{every tick label/.append style={font=\scriptsize}}
\begin{groupplot}[
y tick label style={/pgf/number format/.cd,fixed,precision=2},
scaled y ticks = false,
legend style={at={(1,1)}},
         %title style={at={(0.5,-2.0cm)}, anchor=south},
         title style={at={(0.5,3.35cm)}, anchor=south},
         group
         style={group size= 3 by 1, xlabels at=edge bottom, ylabels at=edge left,yticklabels at=edge left,
           horizontal sep=0.15cm}, xlabel={\scriptsize iteration}, ylabel={\scriptsize MSE},
         width=3.6cm,height=3.6cm, ymin=0,xmin=10]
%%%
	\nextgroupplot[title = {\scriptsize (a) noisy image},xmode=log,ymax=0.025] 
	\addplot +[mark=none] table[x index=0,y index=3]{./figs/DD_denoising_curves.dat};
%	\addlegendentry{\small DD-O}
	
%%%

	\nextgroupplot[title = {\scriptsize (b) clean image},xmode=log]
	\addplot +[mark=none] table[x index=0,y index=1]{./figs/DD_denoising_curves.dat};


	\nextgroupplot[title = {\scriptsize(c)  noise},xmode=log]
	\addplot +[mark=none] table[x index=0,y index=2]{./figs/DD_denoising_curves.dat};

      
\end{groupplot}          

\draw (0.08,2) circle(1.5pt) -- (-0.5cm,2.35cm) node[above,inner sep=-0.5]{
\includegraphics[width=1.1cm]{./figs/phantom256DD_at_10.png}
};

\draw (0.6,0.3) circle(1.5pt) -- (0.7cm,2.35cm) node[above,inner sep=-0.5,draw]{
\includegraphics[width=1.1cm]{./figs/phantom256DD_at_100.png}
};

\draw (1.75,1.25) circle(1.5pt) -- (1.9cm,2.35cm) node[above,inner sep=-0.5]{
\includegraphics[width=1.1cm]{./figs/phantom256DD_at_10000.png}
};

%%%

\draw (4,0) circle(1.5pt) -- (3.5cm,2.35cm) node[above,inner sep=-0.5]{
\includegraphics[width=1.1cm]{./figs/phantom256image_DD_at_10000.png}
};

\draw (6.1,0.25) circle(1.5pt) -- (5.5cm,2.35cm) node[above,inner sep=-0.5]{
\includegraphics[width=1.1cm]{./figs/phantom256noise_DD_at_10000.png}
};
%%%
\end{tikzpicture}
}
\end{center}
\vspace{-0.5cm}
\caption{
\label{fig:fittingcurves}
Fitting an over-parameterized Deep Decoder to a (a) noisy image, (b) clean image, and (c) pure noise. Here, MSE denotes Mean Square Error of the network output with respect to the clean image in (a) and fitted images in (b) and (c). While the network can fit the noise due to over-parameterization, it fits natural images with significantly fewer iterations than noise. Hence, when fitting a noisy image, the image component is fitted faster than the noise component which enables denoising via early stopping.%, hence early stopping denoises.
}
\end{figure}



For denoising, regularization via early stopping is critical for performance, since with enough iterations the network fits the entire noisy image. The early stopping time plays the same role as the number of parameters for image reconstruction with an under-parameterized neural network: More iterations fit the image part better but also fit more of the noise. Fewer iterations fit the image part less well, but also fit less of the noise. 

Empirically, un-trained neural network perform best in the over-parameterized regime. Several variants of convolutional generator networks work well, including the deep decoder, a U-net, and a convolutional generator network~\cite{heckel_DeepDecoderConcise_2019,darestani_AcceleratedMRIUnTrained_2021,ulyanov_DeepImagePrior_2018}. 

\subsubsection{\bf Provable denoising with over-parameterized convolutional networks}
Next, we formalize that convolutional generators optimized with gradient descent fit natural images faster than noise, and show that fitting convolutional generators via early stopped gradient descent provably denoises ``natural'' images. 

We model an image as a smooth signal. We say that a signal $\vx \in \reals^n$ is $p$-smooth if it can be represented as a linear combination of the $p$ first trigonometric basis functions (illustrated in Figure~\ref{fig:circulantsingvectors}). 
Natural images are approximately sparse. For example, \cite[Figure 4]{simoncelli_NaturalImageStatistics_2001} shows that the power spectrum (i.e., the energy distribution by frequency) of a natural
image decays rapidly from low frequencies to high frequencies.



\begin{figure}[t]
\begin{center}
\begin{tikzpicture}
\begin{groupplot}[axis lines=none,
y tick label style={/pgf/number format/.cd,fixed,precision=3},
scaled y ticks = false,
legend style={at={(1.2,1)}},
         title style={at={(0.5,-0.7cm)}, anchor=south}, group
         style={group size= 4 by 1, xlabels at=edge bottom,
           horizontal sep=0.5cm, vertical sep=1.3cm},
         width=3.5cm,height=3cm]

\nextgroupplot[title={$\vw_1$}]
\addplot +[mark=none,thick] table[x index=0,y index=1]{./figs/circulant_singular_vectors.dat};
%\addlegendentry{0}
\nextgroupplot[title={$\vw_2$}]
\addplot +[mark=none,thick] table[x index=0,y index=2]{./figs/circulant_singular_vectors.dat};
\nextgroupplot[title={$\vw_6$}]
%\addlegendentry{1}
\addplot +[mark=none,thick] table[x index=0,y index=3]{./figs/circulant_singular_vectors.dat};
\nextgroupplot[title={$\vw_{21}$}]
%\addlegendentry{5}
\addplot +[mark=none,thick] table[x index=0,y index=4]{./figs/circulant_singular_vectors.dat};
%\addlegendentry{20}
\end{groupplot}          
\end{tikzpicture}
\end{center}
\vspace{-0.5cm}
\caption{
\label{fig:circulantsingvectors}
The 1st, 2nd, 6th, and 21th trigonometric basis functions in dimension $n=300$. 
}
\end{figure}

We consider a randomly initialized network of the form~\eqref{eq:twolayerDD}. 
The following results rely on the insight that the behavior of a large over-parameterized neural networks is dictated
by the spectral properties of their Jacobian mapping at initialization. The left-singular values of the Jacobian of a convolutional network are the trigonometric basis functions $\vw_1,\ldots, \vw_n$. Provided that the fixed convolutional filter of the convolution in the deep decoder network is relatively narrow (which it is in practice), the associated singular values $\sigma_1 > \sigma_2 > \ldots > \sigma_n$ decay rapidly, so that large singular values are associated with low-frequency trigonometric basis functions and small singular values are associated with high-frequency basis functions. 
%The decay of the singular values $\sigma_1,\ldots,\sigma n$ is determined by the fixed convolutional kernel used in the deep decoder: For the popular triangular kernel, the narrower the kernel, the faster the decay of the singular values. 

The following result shows that an un-trained convolutional network fitted with gradient descent, fits the components of the noisy measurement $\vy = \vx + \veta$ that align with the trigonometric basis functions $\vw_1,\ldots, \vw_n$ at speeds determined by associated singular values $\sigma_1 > \sigma_2 > \ldots > \sigma_n$. 

\begin{theorem}[Theorem 2 in \cite{heckel_DenoisingRegularizationExploiting_2020}]
\label{thm:untraineddenoising}
Suppose we fit a randomly initialized network of the form~\eqref{eq:twolayerDD} via applying gradient descent with stepsize $\alpha$ for $t$ iterations to minimizing the least-squares loss $\mathcal L(\vtheta) = \norm{G(\vtheta) - (\vx + \veta) }_2^2$. Here, $\vx$ is a $p$-smooth signal and $\veta$ is an arbitrary noise vector. Suppose that the network is sufficiently wide, i.e., $k \geq O(n/\epsilon^4)$, for some $\epsilon>0$. 
Then the estimate of the un-trained network based on the $t$-th iterate $\vtheta_t$ obeys, with high probability over the random initialization,
\begin{align}
\norm{G(\vtheta_t) - \vx}_2
%
&\leq
(1- \alpha \sigma_p^2)^t \norm{\vx}_2 \nonumber \\
%
&+
\left( \sum_{i=1}^n ( (1-\alpha \sigma_i^2)^t - 1 )^2 \veta^T \vw_i \right)^{1/2} + \epsilon. 
\end{align}
\end{theorem}

In this result, $\epsilon$ is an error that becomes negligible if the network is sufficiently wide. 
The first term is the error for fitting the signal. After sufficiently many iterations for $(1- \alpha \sigma_p^2)^t$ to be small the signal fitting error is small. At the same time, after only sufficiently many iterations for $(1- \alpha \sigma_p^2)^t$ to be small, only the components of the noise that align with the $p$-many lowest frequency trigonometric basis functions are fitted, provided that the singular values decay sufficiently fast. 

A consequence of this result is (see \cite[Theorem 1]{heckel_DenoisingRegularizationExploiting_2020}) that there is an optimal number of iterations so that for denoising a signal corrupted with Gaussian noise $\veta \sim \mathcal N(0,\mI)$, the estimate based on early-stopping the gradient descent iterations obeys 
\begin{align*}
\norm{G(\vtheta_t) - \vx}  \leq O\left( \frac{p}{n}\right).
\end{align*}
This ensures that only a fraction $p/n$ of the noise energy is fitted, and the rest of the noise that lies outside of the signal subspace spanned by the $p$-lowest frequency trigonometric basis functions is filtered out. That is, up to a constant, the best denoising result for denoising a $p$-smooth signal from Gaussian noise that any estimator can yield.

%%%

\subsubsection{\bf Provable signal reconstruction with over-parameterized convolutional networks}

Next, we consider signal reconstruction from $m$ noiseless random measurements, with an un-trained networks via applying gradient descent to the loss~\eqref{eq:untrainedoptprob}. For this setup, perhaps surprisingly, no regularization is necessary since the network has an interesting self-regularization property. 

\begin{theorem}[{Corollary of \cite[Theorem 2]{heckel_CompressiveSensingUntrained_2020}}]
\label{thm:untrainedcs}
Let $\mA \in \reals^{m\times n}$ be a Gaussian random matrix, and suppose we are given noiseless measurements $\vy = \mA \vx$ of a $(m/3)$-smooth signal $\vx$. Consider the two-layer neural network~\eqref{eq:untrainedoptprob}, with kernel chosen so that the singular values of the Jacobian of the network at initialization decay geometrically, i.e., $\sigma_i^2 = \gamma^i$, and suppose the network is sufficiently wide. Then, with high probability, the estimate $\vtheta_\infty$ obtained by apply gradient descent to the loss~\eqref{eq:untrainedoptprob} obeys
\begin{align}
\norm{G(\vtheta_\infty) - \vx}_2^2 \leq O\left( \frac{\gamma^{m/3}}{1-\gamma} \norm{\vx}_2^2 \right).
\end{align}
\end{theorem}

The theorem guarantees almost perfect recovery of a $m/3$-smooth signal from only $m$ measurements, which is optimal up to a constant. 
The mechanism underlying this result is that gradient descent fits the lowest-frequency components of the signal before the higher frequency component, similar to the denoising result in the previous subsection. 

%%%

\subsection{Ongoing Challenges}

The proof of theorems \ref{thm:untraineddenoising} and \ref{thm:untrainedcs} relies on relating the dynamics of gradient descent applied to fitting an over-parameterized network to that of gradient descent of an associated linear network. This proof technique has been used in a variety of recent publications~\cite{soltanolkotabi_TheoreticalInsightsOptimization_2019,du_GradientDescentProvably_2018b,ronen_ConvergenceRateNeural_2019,jacot_NeuralTangentKernel_2018}. 
As such, it is relatively straightforward to extend the analysis to deeper neural networks.

However, the main short coming of the analysis is that it effectively assumes that the network operates in a regime where is behaves essentially like an associated linear model. This is a accurate first order approximation on what un-trained networks do, but in practice un-trained networks do not operate in the regime where they behave like linear models. The behavior that makes un-trained networks work so well compared to linear models for denoising and signal reconstruction cannot be captured by this analysis, and therefore an important avenue for future research is to develop a fine analysis for moderately wide un-trained networks. 


%%%
\subsection{Beyond convolutional un-trained neural networks}

The discussion in this section has focused on image reconstruction with un-trained convolutional neural networks. We end this discussion by noting that un-trained beyond convolutional neural networks are a powerful technique for signal reconstruction beyond images. 

Coordinate-based neural representations for images, 3D shapes, and other signals have recently emerged as an alternative for traditional discrete representations such as sparse representations or convolutional neural networks. 
They have been employed for surface reconstruction~\cite{williams_DeepGeometricPrior_2019}, representing scenes and view synthesis~\cite{mildenhall_NeRFRepresentingScenes_2020}, and for representing and working with images. 
Such networks are un-trained neural networks, as they reconstruct a scene etc without any training, in a similar fashion as the convolutional networks used in this section do.

A key component of many of the coordinate-based neural representations are sinusoidal mappings in the first layer~\cite{mildenhall_NeRFRepresentingScenes_2020,tancik_FourierFeaturesLet_2020a,sitzmann_ImplicitNeuralRepresentations_2020a}. Those networks are very related to convolutional un-trained neural networks, since they can be shown to be equivalent to convolutional architectures if sufficiently wide. 

Finally, un-trained neural networks have also been used to reconstruct graph signals~\cite{rey_UntrainedGraphNeural_2021}, as well as continuously indexed objects through fitting probabilistic models~\cite{zhong_ReconstructingContinuousDistributions_2020,rosenbaum_InferringContinuousDistribution_2021}. 





